DISCO: Efficient Diffusion Solver for Large-Scale Combinatorial Optimization Problems

Combinatorial Optimization (CO) problems are fundamentally important in numerous real-world applications across diverse industries, characterized by entailing enormous solution space and demanding time-sensitive response. Despite recent advancements in neural solvers, their limited expressiveness struggles to capture the multi-modal nature of CO landscapes. While some research has shifted towards diffusion models, these models still sample solutions indiscriminately from the entire NP-complete solution space with time-consuming denoising processes, which limit their practicality for large problem scales. We propose DISCO, an efficient DIffusion Solver for large-scale Combinatorial Optimization problems that excels in both solution quality and inference speed. DISCO's efficacy is twofold: First, it enhances solution quality by constraining the sampling space to a more meaningful domain guided by solution residues, while preserving the multi-modal properties of the output distributions. Second, it accelerates the denoising process through an analytically solvable approach, enabling solution sampling with minimal reverse-time steps and significantly reducing inference time. DISCO delivers strong performance on large-scale Traveling Salesman Problems and challenging Maximal Independent Set benchmarks, with inference time up to 5.28 times faster than other diffusion alternatives. By incorporating a divide-and-conquer strategy, DISCO can well generalize to solve unseen-scale problem instances, even surpassing models specifically trained for those scales.

==> tables/ablation.tex <==

\begin{table}[h]
    \setlength{\tabcolsep}{3pt}
    \caption{Ablation results on model components. R denotes residual constraints. \zh{Waiting for larger scale experiments.}
    }
    \label{tab:ablation}
    \vspace{-0.1in}
    \begin{center}
    \begin{small}
    \begin{sc}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l|c|c|ccc|ccc}
    \toprule
    \multirow{2}*{Algorithm}& \multirow{2}*{Type}& \multirow{2}*{Steps} & \multicolumn{3}{c}{TSP-50} & \multicolumn{3}{|c}{TSP-100}\\
     &  & & Length$\downarrow$ & Gap(\%)$\downarrow$ & Time $\downarrow$ &Length $\downarrow$ & Gap(\%)$\downarrow$ & Time $\downarrow$ \\
     \midrule
     DIFUSCO & Greedy & 2 & 5.77 & 1.40 & 0.23$\mathrm{m}$ & 
     8.00 & 3.06 & 0.84 $\mathrm{m}$\\
     DIFUSCO & Greedy & 50 & 5.70 & 0.10 & 4.86$\mathrm{m}$ &
     7.78 & 0.24 & 10.80 $\mathrm{m}$\\
     \method{} w/o R & Greedy &  2 & 5.72 & 0.55  &  0.21 $\mathrm{m}$ 
       & &   \\
     \method{} (\textbf{Ours}) & Greedy &  2 & 5.70 & 0.21 & 0.39 $\mathrm{m}$ &
      7.82 & 0.81 & 0.73 $\mathrm{m}$ \\
     \method{} (\textbf{Ours}) & Greedy &  1 & 5.70 & 0.16 & 0.24 $\mathrm{m}$ & 
      7.81 & 0.59 & 0.45 $\mathrm{m}$ \\
     
    \midrule
    DIFUSCO & $16\times$Sampling & 2 & 5.69 & 0.00 & 1.82 $\mathrm{m}$ &
    7.78 & 0.28 & 7.55 $\mathrm{h}$ \\
    DIFUSCO & $16\times$Sampling & 50 & 5.69 & -0.01 & 33.34 $\mathrm{m}$ & 
    7.76 & -0.02 & 2.05 $\mathrm{h}$ \\
    % ResDCO w/o A & $16\times$Sampling &  10 & \textbf{} & \textbf{} & \textbf{} & \textbf{} \\
    \method{} w/o R & $16\times$Sampling &  2 & 5.69 & -0.01 & 2.16 $\mathrm{m}$ &  &  & \\
    \method{} (\textbf{Ours}) & $16\times$Sampling &  2 & 5.69 & -0.01 & 1.92 $\mathrm{m}$ & 7.76 & 0.03 & 6.25 $\mathrm{m}$ \\
    \method{} (\textbf{Ours}) & $16\times$Sampling &  1 & 5.70 & 0.18 & 1.43 $\mathrm{m}$ & 7.81 & 0.62 & 3.56 $\mathrm{m}$ \\

    \bottomrule
    \end{tabular}
    }
    \end{sc}
    \end{small}
    \end{center}
    \vskip -0.1in
    \setlength{\tabcolsep}{6pt}
  \end{table}


==> tables/all_one_single_step.tex <==
\begin{table}[h]
    \caption{Comparisons of diffusion-based methods with all denoise step set to one.
          }
    \label{tab:all_one_denoise_step_comp}
    \begin{sc}
    \begin{center}
    \small
    \centering
    \resizebox{0.5\textwidth}{!}{
    \begin{tabular}{ll|ccccccccc}
    \toprule
    % \multirow{2}*{Algorithm}&\multirow{2}*{Type} 
    % &\multicolumn{2}{c|}{N(0.5, 0.1)}&\multicolumn{2}{c|}{U(0.1, 0.9)}&\multicolumn{2}{c}{Cluster}\\
    Algorithm & Type 
    &Length $\downarrow$&Gap $\downarrow$&Time $\downarrow$\\
    \midrule
    DIFUSCO   & SL+G$\dag$ 
    & 77.84 & 8.46\% & 26.68$\mathrm{m}$ 
    \\
    T2T   & SL+G$\dag$ 
    & 77.49 & 7.97\% & 70.80$\mathrm{m}$ 
    \\
    \method{}   & SL+G$\dag$ 
    & \textbf{73.85} & \textbf{2.89\%} & 25.12$\mathrm{m}$ 
    \\
    \bottomrule
    \end{tabular}
    }
    \end{center}
    \end{sc}
    \vspace{-6pt}
    \end{table}

==> tables/error_bar.tex <==
\begin{table}[!h]
    \caption{Statistical analysis of 
    repeated evaluations on large-scale TSP problems. MS denotes our multi-modality inspired graph search method,  where each search samples 50 solution trials.}
    % \vspace{-10pt}
    \label{tab:statistical_analysis}
    \begin{sc}
    \begin{center}
    \small
    \centering
    \resizebox{1\textwidth}{!}{
    \begin{tabular}{ll|ccc|ccc|ccc}
    \toprule
    \multirow{2}*{Algorithm}&\multirow{2}*{Type}%
    &\multicolumn{3}{c|}{TSP-500}&\multicolumn{3}{c|}{TSP-1000}&\multicolumn{3}{c}{TSP-10000}\\
    &&Length $\downarrow$&Std $\downarrow$&Time $\downarrow$&Length $\downarrow$&Std $\downarrow$&Time $\downarrow$&Length $\downarrow$&Std $\downarrow$&Time $\downarrow$\\
    \midrule
    % DIFUSCO   & SL+G$\dag$+2-opt & 16.800$\pm 0.002$ & $4.06\times10^{-3}$ & 3.65$\mathrm{m}$ & 23.560$\pm 0.011$ & $7.43\times10^{-3}$ & 12.06$\mathrm{m}$ & & & 
    % \\
    \method{}   & SL+G$\dag$+2-opt
    & 16.862$\pm 0.008$ & $4.81\times10^{-2}$ & 0.25$\mathrm{m}$
    & 23.653$\pm 0.005$ & $2.92\times10^{-3}$ & 1.12$\mathrm{m}$
    & 73.851$\pm 0.035$ & $3.00\times10^{-2}$ & 25.12$\mathrm{m}$
    \\
    % \midrule
    % DIFUSCO   &  SL+S+2-opt
    % & 16.656$\pm 0.005$ & $3.71\times10^{-3}$ & 11.46$\mathrm{m}$ 
    % & 23.451$\pm 0.005$ & $3.53\times10^{-3}$ & 48.09$\mathrm{m}$
    % &  &  & 
    % \\
    \method{}   &  SL+S+2-opt
    & 16.733$\pm 0.002$ & $1.14\times10^{-3}$ & 3.88$\mathrm{m}$
    & 23.651$\pm 0.007$ & $5.77\times10^{-3}$ & 9.62$\mathrm{m}$
    & 73.811$\pm 0.031$ & $3.51\times10^{-2}$ & 1.60\textbf{$\mathrm{h}$}
    \\
    % \midrule
    % DIFUSCO  & SL+MCTS
    % & 
    % \\
    % \midrule
    \method{}   & SL+MCTS
    & 16.632$\pm 0.004$ & $2.68\times10^{-3}$  & 6.99$\mathrm{m}$ 
    & 23.419$\pm 0.004$ & $2.91\times10^{-3}$  & 15.82$\mathrm{m}$
    & 73.562$\pm 0.029$ & $3.27\times10^{-2}$  & 42.35$\mathrm{m}$
    % \\
    % \midrule
    % DIFUSCO + MS  & SL+G$\dag$+2-opt & 
    \\
    \method{} + MS  & SL+G$\dag$+2-opt 
    & 16.789$\pm 0.005$ &  $3.49\times10^{-3}$ & 11.67$\mathrm{m}$ 
    & 23.614$\pm 0.003$ & $2.51\times10^{-3}$ & 28.83$\mathrm{m}$
    & 74.240$\pm 0.034$ & $3.21\times10^{-2}$ & 1.82$\mathrm{h}$ 
    \\
    \bottomrule
    \end{tabular}
    }
    \end{center}
    \end{sc}
    \vspace{-10pt}
    \end{table}

==> tables/graph_fusion.tex <==
\begin{algorithm}[h]
	\caption{Multi-Modal Graph Fusion}
	\renewcommand{\algorithmicrequire}{ \textbf{Input:}}
	\renewcommand{\algorithmicensure}{ \textbf{Process:}}
	\label{alg:framework}
	\begin{algorithmic}[1]
		\REQUIRE A large-scale graph problem $G$ to be solved. 
		\ENSURE
		\STATE Pre-train \method{} model $p_\theta$ on small-scale instances. 
        \STATE Sample a set of subgraphs $\mathbf{g}$ from $G$.
		\FOR{$g \in \mathbf{g}$}
        \STATE Sample heatmap set $\mathbf{h}$  from $p_\theta(g)$ with $q$ different noise $\mathbf{x}^\mathbf{T}.$
        \ENDFOR
        \FOR{$k = 1, 2, 3, ..., n$}
            \STATE Sample $h$ from each $\mathbf{h}$ as combination $\mathbf{c}_k$. 
            \STATE Decode solution $\mathbf{x}_k$ from $\mathbf{c}_k$ and add it to trial set $\mathcal{X}$.
        \ENDFOR
		\STATE 
        Select the best trial with $\argmin_{\mathbf{x}\in \mathcal{X}} cost(\mathbf{x})$.
		\label{alg:fusion}
    \end{algorithmic}
\end{algorithm}



==> tables/image_denoising_tsp_100.tex <==

\begin{figure}[!h]
    \centering
    \vspace{-2mm}
    % 包裹所有 subfigure 的 minipage
    \begin{minipage}{1\linewidth}
        \centering
        \subfigure{
            \includegraphics[width=0.145\linewidth, clip, trim=50 60 50 60]{images/denoising_fig/ddim/tsp100-inf5/val-0-step-0.png}
        }
        \subfigure{        
            \includegraphics[width=0.145\linewidth, clip, trim=50 60 50 60]{images/denoising_fig/ddim/tsp100-inf5/val-0-step-1.png}
        }
        \subfigure{
            \includegraphics[width=0.145\linewidth, clip, trim=50 60 50 60]{images/denoising_fig/ddim/tsp100-inf5/val-0-step-2.png}
        }
        \subfigure{
            \includegraphics[width=0.145\linewidth, clip, trim=50 60 50 60]{images/denoising_fig/ddim/tsp100-inf5/val-0-step-3.png}
        }
        \subfigure{
            \includegraphics[width=0.145\linewidth, clip, trim=50 60 50 60]{images/denoising_fig/ddim/tsp100-inf5/val-0-step-4.png}
        }
        \subfigure{
            \includegraphics[width=0.145\linewidth, clip, trim=50 60 50 60]{images/denoising_fig/ddim/tsp100-inf5/val-0-step-5.png}
        }
        % \vspace{-10pt}
        \subfigure{
            \includegraphics[width=0.145\linewidth, clip, trim=50 60 50 60]{images/denoising_fig/ddm/tsp100-inf5/val-0-step-0.png}
        }
        \subfigure{        
            \includegraphics[width=0.145\linewidth, clip, trim=50 60 50 60]{images/denoising_fig/ddm/tsp100-inf5/val-0-step-1.png}
        }
        \subfigure{
            \includegraphics[width=0.145\linewidth, clip, trim=50 60 50 60]{images/denoising_fig/ddm/tsp100-inf5/val-0-step-2.png}
        }
        \subfigure{
            \includegraphics[width=0.145\linewidth, clip, trim=50 60 50 60]{images/denoising_fig/ddm/tsp100-inf5/val-0-step-3.png}
        }
        \subfigure{
            \includegraphics[width=0.145\linewidth, clip, trim=50 60 50 60]{images/denoising_fig/ddm/tsp100-inf5/val-0-step-4.png}
        }
        \subfigure{
            \includegraphics[width=0.145\linewidth, clip, trim=50 60 50 60]{images/denoising_fig/ddm/tsp100-inf5/val-0-step-5.png}
        }
        % \vspace{-10pt}
        \subfigure{
            \includegraphics[width=0.145\linewidth, clip, trim=50 60 50 60]{images/denoising_fig/rddm/tsp100-inf5/val-0-step-0.png}
        }
        \subfigure{        
            \includegraphics[width=0.145\linewidth, clip, trim=50 60 50 60]{images/denoising_fig/rddm/tsp100-inf5/val-0-step-1.png}
        }
        \subfigure{
            \includegraphics[width=0.145\linewidth, clip, trim=50 60 50 60]{images/denoising_fig/rddm/tsp100-inf5/val-0-step-2.png}
        }
        \subfigure{
            \includegraphics[width=0.145\linewidth, clip, trim=50 60 50 60]{images/denoising_fig/rddm/tsp100-inf5/val-0-step-3.png}
        }
        \subfigure{
            \includegraphics[width=0.145\linewidth, clip, trim=50 60 50 60]{images/denoising_fig/rddm/tsp100-inf5/val-0-step-4.png}
        }
        \subfigure{
            \includegraphics[width=0.145\linewidth, clip, trim=50 60 50 60]{images/denoising_fig/rddm/tsp100-inf5/val-0-step-5.png}
        }
    \end{minipage}
    \put(-400, 70){\rotatebox{90}{\makebox(0,0){\small  DIFFUSCO}}}
    \put(-400, 0){\rotatebox{90}{\makebox(0,0){\small  DDM}}}
    \put(-400, -65){\rotatebox{90}{\makebox(0,0){\small  Ours}}}
    \put(-356, -100){\makebox(0,0){\small  Step 0}}
    \put(-292, -100){\makebox(0,0){\small  Step 1}}
    \put(-226, -100){\makebox(0,0){\small  Step 2}}
    \put(-163, -100){\makebox(0,0){\small  Step 3}}
    \put(-96, -100){\makebox(0,0){\small   Step 4}}
    \put(-33,  -100){\makebox(0,0){\small  Step 5}}
    \caption{Denoising process on TSP-100.}
    \label{fig:denoising_tsp_100}
\end{figure}


==> tables/image_denoising_tsp_500.tex <==
\begin{figure}[!h]
    \centering
    \vspace{-2mm}
    % 包裹所有 subfigure 的 minipage
    \begin{minipage}{1\linewidth}
        \centering
        \subfigure{
            \includegraphics[width=0.145\linewidth, clip, trim=50 60 50 60]{images/denoising_fig/ddim/tsp500-inf5/val-0-step-0.png}
        }
        \subfigure{        
            \includegraphics[width=0.145\linewidth, clip, trim=50 60 50 60]{images/denoising_fig/ddim/tsp500-inf5/val-0-step-1.png}
        }
        \subfigure{
            \includegraphics[width=0.145\linewidth, clip, trim=50 60 50 60]{images/denoising_fig/ddim/tsp500-inf5/val-0-step-2.png}
        }
        \subfigure{
            \includegraphics[width=0.145\linewidth, clip, trim=50 60 50 60]{images/denoising_fig/ddim/tsp500-inf5/val-0-step-3.png}
        }
        \subfigure{
            \includegraphics[width=0.145\linewidth, clip, trim=50 60 50 60]{images/denoising_fig/ddim/tsp500-inf5/val-0-step-4.png}
        }
        \subfigure{
            \includegraphics[width=0.145\linewidth, clip, trim=50 60 50 60]{images/denoising_fig/ddim/tsp500-inf5/val-0-step-5.png}
        }
        % \vspace{-10pt}
        \subfigure{
            \includegraphics[width=0.145\linewidth, clip, trim=50 60 50 60]{images/denoising_fig/ddim/tsp500-inf5/val-0-step-0.png}
        }
        \subfigure{        
            \includegraphics[width=0.145\linewidth, clip, trim=50 60 50 60]{images/denoising_fig/ddim/tsp500-inf5/val-0-step-1.png}
        }
        \subfigure{
            \includegraphics[width=0.145\linewidth, clip, trim=50 60 50 60]{images/denoising_fig/ddim/tsp500-inf5/val-0-step-2.png}
        }
        \subfigure{
            \includegraphics[width=0.145\linewidth, clip, trim=50 60 50 60]{images/denoising_fig/ddim/tsp500-inf5/val-0-step-3.png}
        }
        \subfigure{
            \includegraphics[width=0.145\linewidth, clip, trim=50 60 50 60]{images/denoising_fig/ddim/tsp500-inf5/val-0-step-4.png}
        }
        \subfigure{
            \includegraphics[width=0.145\linewidth, clip, trim=50 60 50 60]{images/denoising_fig/ddim/tsp500-inf5/val-0-step-5.png}
        }
        % \vspace{-10pt}
        \subfigure{
            \includegraphics[width=0.145\linewidth, clip, trim=50 60 50 60]{images/denoising_fig/rddm/tsp500-inf5/val-0-step-0.png}
        }
        \subfigure{        
            \includegraphics[width=0.145\linewidth, clip, trim=50 60 50 60]{images/denoising_fig/rddm/tsp500-inf5/val-0-step-1.png}
        }
        \subfigure{
            \includegraphics[width=0.145\linewidth, clip, trim=50 60 50 60]{images/denoising_fig/rddm/tsp500-inf5/val-0-step-2.png}
        }
        \subfigure{
            \includegraphics[width=0.145\linewidth, clip, trim=50 60 50 60]{images/denoising_fig/rddm/tsp500-inf5/val-0-step-3.png}
        }
        \subfigure{
            \includegraphics[width=0.145\linewidth, clip, trim=50 60 50 60]{images/denoising_fig/rddm/tsp500-inf5/val-0-step-4.png}
        }
        \subfigure{
            \includegraphics[width=0.145\linewidth, clip, trim=50 60 50 60]{images/denoising_fig/rddm/tsp500-inf5/val-0-step-5.png}
        }
    \end{minipage}
    \put(-400, 70){\rotatebox{90}{\makebox(0,0){\small  DIFFUSCO}}}
    \put(-400, 0){\rotatebox{90}{\makebox(0,0){\small  \zh{\method{} w/o R}}}}
    \put(-400, -65){\rotatebox{90}{\makebox(0,0){\small  \method{} (Ours)}}}
    \put(-356, -100){\makebox(0,0){\small  Step 0}}
    \put(-292, -100){\makebox(0,0){\small  Step 1}}
    \put(-226, -100){\makebox(0,0){\small  Step 2}}
    \put(-163, -100){\makebox(0,0){\small  Step 3}}
    \put(-96, -100){\makebox(0,0){\small   Step 4}}
    \put(-33,  -100){\makebox(0,0){\small  Step 5}}
    \caption{Denoising processes on TSP-500.}
    \label{fig:denoising_tsp_500}
\end{figure}


==> tables/image_diffusion_sample.tex <==
\begin{figure}[h]
    \centering
    \hfill
    % \subfigure[Performance of baseline.]{
    \subfigure{
        \includegraphics[width=0.31\linewidth]{images/color_map/ddim_gaps.pdf}
        }
    \hfill
    % \subfigure[Performance of \method.]{
    \subfigure{
        \includegraphics[width=0.31\linewidth]{images/color_map/rddm_gaps.pdf}
    }
    \hfill
    % \subfigure[Runtime of \method.]{
    \subfigure{
        \includegraphics[width=0.31\linewidth]{images/color_map/rddm_times.pdf}
    }
    \hfill
    \put(-330, -3){\makebox(0,0){\small  (a) Performance of baseline.}}
    \put(-198, -3){\makebox(0,0){\small  (b) Performance of \method.}}
    \put(-65, -3){\makebox(0,0){\small   (c) Runtime of \method.}}
    \caption{The performance of both the baseline method DIFUSCO \citep{DIFUSCO} (a) and \method{} (b)  on TSP-50 instances with different denoising steps and sample number. Corresponding per-instance run-time ($\mathrm{sec}$) of diffusion-based methods is depicted in (c).
    The negative performance gap arises because the Concorde solver, used for providing labels, only accepts integer coordinates as inputs, resulting in inaccurate non-optimal solutions due to rounding issues. 
     For \method{} with a denoising step of 1, its variance $\sigma$ tends to zero, as described by Eq.~\ref{eq8}, yielding relatively more confident solutions and potentially better performance.
     However, this does not lead to performance improvement in response to actively sampling more times.
    \label{fig:diffusion_sample}
     }
    \vspace{-6pt}
\end{figure}


==> tables/inference_advantage.tex <==

\begin{table}[h]
    \setlength{\tabcolsep}{3pt}
    \caption{Results on multi modal inference.}
    \label{tab:tsp50-100}
    \vspace{-0.1in}
    \begin{center}
    \begin{small}
    \begin{sc}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lccccc}
    \toprule
    \multirow{2}*{Algorithm}& \multirow{2}*{Type}& \multicolumn{2}{c}{TSP-50} & \multicolumn{2}{c}{TSP-100}\\
     &  & Length$\downarrow$ & Gap(\%)$\downarrow$ & Length $\downarrow$ & Gap(\%)$\downarrow$ \\
    \midrule
    Concorde$^*$ & Exact & 5.69 & 0.00 & 7.76 & 0.00\\
    2-OPT & Heuristics & 5.86 & 2.95 & 8.03 & 3.54\\
    \midrule
    ResDCO & $1\times$Sampling & \textbf{} & \textbf{} & \textbf{} & \textbf{} \\
    ResDCO & $2\times$Sampling & \textbf{} & \textbf{} & \textbf{} & \textbf{} \\
    ResDCO & $4\times$Sampling & \textbf{} & \textbf{} & \textbf{} & \textbf{} \\
    ResDCO & $8\times$Sampling & \textbf{} & \textbf{} & \textbf{} & \textbf{} \\
    ResDCO & $16\times$Sampling & \textbf{} & \textbf{} & \textbf{} & \textbf{} \\
    \bottomrule
    \end{tabular}
    }
    \end{sc}
    \end{small}
    \end{center}
    \vskip -0.1in
    \setlength{\tabcolsep}{6pt}
    \end{table}


==> tables/mis.tex <==
\begin{table}[h]
\label{tab:mis}
\caption{Results on MIS problems.}
% \vspace{-0.1in}
\begin{center}
\resizebox{0.6\textwidth}{!}{
\begin{tabular}{l |c |ccc |ccc}
    \toprule
    \multirow{2}*{Method}&\multirow{2}*{Type}
    &\multicolumn{3}{c|}{SATLIB}&\multicolumn{3}{c}{ER-[700-800]}\\
    &&Size $\uparrow$&Gap $\downarrow$&Time $\downarrow$&Size $\uparrow$&Gap $\downarrow$&Time $\downarrow$ \\
    \midrule
    KaMIS&Heuristics
    &425.96$^*$&---&37.58$\mathrm{m}$ &44.87$^*$&---&52.13$\mathrm{m}$ \\
    Gurobi&Exact &
    425.95& 0.00\%& 26.00$\mathrm{m}$ &  41.38 & 7.78\% & 50.00$\mathrm{m}$ \\
    \midrule
    Intel & SL+G & 420.66 & 1.48\% & 23.05$\mathrm{m}$ & 34.86 & 22.31\% & 6.06$\mathrm{m}$ \\
    Intel & SL+TS & N/A & N/A & N/A & 38.80 & 13.43\% & 20.00m  \\
    DGL   & SL+TS & N/A & N/A & N/A & 37.26 & 16.96\% & 22.71$\mathrm{m}$ \\
    LwD & RL+S & 422.22 & 0.88\% & 18.83$\mathrm{m}$ & 41.17 & 8.25\% & 6.33$\mathrm{m}$ \\
    DIMES &RL+G& 421.24 & 1.11\% & 24.17$\mathrm{m}$ & 38.24 & 14.78\% & 6.12$\mathrm{m}$ \\
    DIMES &RL+S& 423.28 & 0.63\% & 20.26$\mathrm{m}$ & \textbf{42.06} & \textbf{6.26\%} & 12.01$\mathrm{m}$ \\
    DIFUSCO & SL+G & \textbf{} & \textbf{} &  &  &  & \\
    DIFUSCO & SL+S & \textbf{} & \textbf{} &  &  &  & \\
    \midrule
    \method{} (\textbf{Ours}) & SL+G & \textbf{} & \textbf{} &  &  &  & 
    \\
    \method{} (\textbf{Ours}) & SL+S  & \textbf{} & \textbf{} &  &  &  & 
    \\
    \bottomrule
\end{tabular}
}
\end{center}
\end{table}




==> tables/multi_modal.tex <==

\begin{table}[h]
    \setlength{\tabcolsep}{3pt}
    \caption{Multi modal inference on TSP-50 and TSP-100.}
    \label{tab:tsp50-100}
    \vspace{-0.1in}
    \begin{center}
    \begin{small}
    \begin{sc}
    \resizebox{0.8\linewidth}{!}{
    \begin{tabular}{lccccccc}
    \toprule
    \multirow{2}*{Algorithm}& \multirow{2}*{Type}& \multicolumn{2}{c}{TSP-50} & \multicolumn{2}{c}{TSP-100}\\
     &  & Length$\downarrow$ & Gap(\%)$\downarrow$ & Length $\downarrow$ & Gap(\%)$\downarrow$ \\
    \midrule
    Concorde$^*$ & Exact & 5.69 & 0.00 & 7.76 & 0.00\\
    2-OPT & Heuristics & 5.86 & 2.95 & 8.03 & 3.54\\
    \midrule
    ResDCO & $1\times$Sampling & \textbf{} & \textbf{} & \textbf{} & \textbf{} \\
    ResDCO & $2\times$Sampling & \textbf{} & \textbf{} & \textbf{} & \textbf{} \\
    ResDCO & $4\times$Sampling & \textbf{} & \textbf{} & \textbf{} & \textbf{} \\
    ResDCO & $8\times$Sampling & \textbf{} & \textbf{} & \textbf{} & \textbf{} \\
    ResDCO & $16\times$Sampling & \textbf{} & \textbf{} & \textbf{} & \textbf{} \\
    \bottomrule
    \end{tabular}
    }
    \end{sc}
    \end{small}
    \end{center}
    \vskip -0.1in
    \setlength{\tabcolsep}{6pt}
    \end{table}


==> tables/no_decoding.tex <==
% \begin{table}[!h]
%     \caption{Performance comparison without decoding strategies.}
%     % \vspace{-10pt}
%     \label{tab:no_decoding}
%     \begin{sc}
%     \begin{center}
%     \small
%     \centering
%     \resizebox{1\textwidth}{!}{
%     \begin{tabular}{ll|c|ccc|ccc|ccc}
%     \toprule
%     \multirow{2}*{Algorithm}&\multirow{2}*{Type}&\multirow{2}*{Steps}%
%     &\multicolumn{3}{c|}{TSP-500}&\multicolumn{3}{c|}{TSP-1000}&\multicolumn{3}{c}{TSP-10000}\\
%     &&&Length $\downarrow$&Gap $\downarrow$&Time $\downarrow$&Length $\downarrow$&Gap $\downarrow$&Time $\downarrow$&Length $\downarrow$&Gap $\downarrow$&Time $\downarrow$\\
%     \midrule
%     LKH-3 (default)& Heuristics & ---
%     &16.55$^*$&0.00\%&46.28$\mathrm{m}$
%     &23.12$^*$&0.00\%&2.57$\mathrm{h}$
%     &71.77$^*$&---&8.8$\mathrm{h}$
%     \\
%     \midrule
%     DIFUSCO   & SL+G & 50
%     & 18.35 & 10.85\% & 3.61$\mathrm{m}$
%     & 26.14 & 13.06\% & 11.86$\mathrm{m}$
%     & 98.15 & 36.75\% & 28.51$\mathrm{m}$
%     \\
%     \method{}   & SL+G & 50
%     & 18.87 & 14.02\% & 4.11$\mathrm{m}$
%     & 27.32 & 18.17\% & 10.47$\mathrm{m}$
%     & 136.80& 90.61\% & 27.40$\mathrm{m}$
%     \\
%     \midrule
%     DIFUSCO   & SL+G & 5
%     & 20.75 & 25.38\% & 0.50$\mathrm{m}$
%     & 30.96 & 33.91\% & 1.88$\mathrm{m}$
%     & 101.60& 41.56\% & 10.05$\mathrm{m}$
%     \\
%     \method{}   & SL+G & 5
%     & 19.25  & 16.31\%  & 0.50$\mathrm{m}$ 
%     & 29.86  & 29.15\%  & 2.12$\mathrm{m}$
%     & 167.35 & 133.18\% & 8.67$\mathrm{m}$
%     \\
%     % DIFUSCO   &  SL+S+2-opt
%     % & 
%     % \\
%     % \method{}   &  SL+S+2-opt
%     % & 16.757 &  $5.22\times10^{-3}$ & 5.17$\mathrm{m}$
%     % & 23.651 & $5.77\times10^{-3}$ & 9.62$\mathrm{m}$
%     % & 73.801 & $3.51\times10^{-2}$ & 1.67\textbf{$\mathrm{h}$}
%     % \\
%     % \midrule
%     % DIFUSCO   & SL+MCTS
%     % & 
%     % \\
%     % \method{}   & SL+MCTS
%     % & 16.680 & $3.64\times10^{-3}$  & 7.38$\mathrm{m}$ 
%     % & 23.419 &  $2.91\times10^{-3}$ & 15.82$\mathrm{m}$
%     % & 73.562 & $3.27\times10^{-2}$  & 42.35$\mathrm{m}$
%     % \\
%     % \midrule
%     % DIFUSCO   & SL+G$\dag$+2-opt
%     % \\
%     % \method{}  & SL+G$\dag$+2-opt 
%     % & 16.789 &  $3.49\times10^{-3}$ & 11.67$\mathrm{m}$ 
%     % & 23.616 & $4.55\times10^{-3}$ & 28.83$\mathrm{m}$
%     % & 74.240 & $3.21\times10^{-2}$ & 1.82$\mathrm{h}$ 
%     % \\
%     \bottomrule
%     \end{tabular}
%     }
%     \end{center}
%     \end{sc}
%     \vspace{-10pt}
%     \end{table}
